Convex X-ray Spectra of PKS 2155-304 and Constraints on the Minimum Electron Energy

The convex (concave upward) high-energy X-ray spectra of the blazar PKS\,2155-304, observed by \emph{XMM-Newton}, is interpreted as the signature of sub-dominant inverse Compton emission. The spectra can be well fitted by a superposition of two power-law contributions which imitate the emission due to synchrotron and inverse Compton processes. The methodology adopted enables us to constrain the photon energy down to a level where inverse Compton emission begins to contribute. We show that this information supplemented with knowledge of the jet Doppler factor and magnetic field strength can be used to constrain the low-energy cutoff $\gamma_{\rm min}m_{\rm e} c^2$ of the radiating electron distribution and the kinetic power $P_{\rm j}$ of the jet. We deduce these quantities through a statistical fitting of the broadband spectral energy distribution of PKS\,2155-304 assuming synchrotron and synchrotron self Compton emission mechanisms. Our results favour a minimum Lorentz factor for the non-thermal electron distribution of $\gamma_{\rm min} \gtrsim 60$, with a preference for a value around $\gamma_{\rm min} \simeq 330$. The required kinetic jet power is of the order of $P_{\rm j} \sim 3\times 10^{45}$ erg s$^{-1}$ in case of a heavy, electron-proton dominated jet, and could be up to an order of magnitude less in case of a light, electron-positron dominated jet. When put in context, our best fit parameters support the X-ray emitting part of blazar jets to be dominated by an electron-proton rather than an electron-positron composition.

==> README <==
% readme.txt
%
% MNRAS journal LaTeX package
% v3.0 for LaTeX 2e
%
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `author-maintained'.
% 
% The Current Maintainer of this work is: Royal Astronomical Society,
% MNRAS Editorial Office, who can be contacted on mn@ras.org.uk
%
% This work consists of all the files listed in readme.txt
%
%
% Last updated 22 May 2015
%
% Copyright (C) Royal Astronomical Society 2015, Blackwell Science 2001,
% Cambridge University Press 1994
%
% See each file for a detailed author list and change log.
%
% This package consists of the following files:

readme.txt          This file

mnras.cls           MNRAS LaTeX document class
mnras.bst           MNRAS BibTeX style

mnras_guide.tex     User guide, LaTeX format
mnras_guide.pdf     User guide, PDF format
mnras_template.tex  A simple template paper

example.eps         An example image used in the guide
example.png         An example image used in the guide
example.ps          An example image used in the guide

legacy\legacy.txt   Description of the legacy releases
legacy\mn2e.cls     v2.2 of mn2e.cls (deprecated)
legacy\mn2e.bst     v1.1b of mn2e.bst (deprecated)


% Disclaimer:
%
% This LaTeX package is provided free to the community in the hope that it
% assists them in preparing papers for the journal Monthly Notices of the
% Royal Astronomical Society.
% The files are provided 'as-is' with no guarantee of their suitability,
% freedom from errors or omissions, or compatibility with any software.
% The Royal Astronomical Society cannot provide user support for this package,
% LaTeX, or for any other software.
% Authors are free to use other styles or programmes if they wish.
% Please see the journal instructions to authors for guidance.
% This disclaimer is in addition to the No Warranty section of the licence,
% at the link given above.
